On Learning Prediction-Focused Mixtures

Probabilistic models help us encode latent structures that both model the data and are ideally also useful for specific downstream tasks. Among these, mixture models and their time-series counterparts, hidden Markov models, identify discrete components in the data. In this work, we focus on a constrained capacity setting, where we want to learn a model with relatively few components (e.g. for interpretability purposes). To maintain prediction performance, we introduce prediction-focused modeling for mixtures, which automatically selects the dimensions relevant to the prediction task. Our approach identifies relevant signal from the input, outperforms models that are not prediction-focused, and is easy to optimize; we also characterize when prediction-focused modeling can be expected to work.

==> figures/results-table-new.tex <==
\newcommand{\msd}[2]{{\small #1}{\tiny (#2)}}
\newcommand{\bmsd}[2]{\textbf{\small #1}{\tiny (#2)}}

% \begin{table*}[t]
% \centering
% \begin{tabular}{@{}l cc cc cc cc cc l@{}}
% \toprule
%  & \multicolumn{4}{c}{Total Dimensions, $D$ = 10} & \multicolumn{6}{c}{Total Dimensions, $D$ = 100}
% \\\cmidrule(lr){2-5}\cmidrule(lr){6-11}
%  & \multicolumn{2}{c}{\drel = 5} & \multicolumn{2}{c}{\drel = 2} & \multicolumn{2}{c}{\drel = 50} & \multicolumn{2}{c}{\drel = 10} & \multicolumn{2}{c}{\drel = 2}
% \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
%  & \mugap=6 & \mugap=8 & \mugap=6 & \mugap=8 & \mugap=6 & \mugap=8 & \mugap=6 & \mugap=8 & \mugap=6 & \mugap=8 
% \\ \midrule 

% {\small \textsc{2-Step}}& \bmsd{0.9}{0.0} & \bmsd{1.1}{0.1} & \msd{3.1}{0.1} & \msd{3.0}{0.1}& \bmsd{1.1}{0.0} & \msd{3.1}{0.1} & \msd{3.1}{0.1} & \msd{3.1}{0.1} & \bmsd{3.1}{0.1} & \msd{3.0}{0.1} \\

 
% {\small \textsc{GMM}}& \bmsd{0.9}{0.1} & \msd{3.1}{0.1} & \msd{3.1}{0.1} & \msd{3.0}{0.1}& \bmsd{1.1}{0.1} & \msd{3.1}{0.1} & \msd{3.1}{0.1} & \msd{3.2}{0.1} & \bmsd{3.2}{0.1} & \msd{3.0}{0.1} \\

% {\small \pfMM-\textsc{AltLB}}& \msd{1.0}{0.0} & \bmsd{1.1}{0.1} & \bmsd{1.2}{0.1} & \msd{1.2}{0.0}& - & - & - & - & - & - \\

% {\small \pfMM-\textsc{\loglike}}& \bmsd{0.9}{0.1} & \bmsd{1.1}{0.1} & \bmsd{1.0}{0.1} & \msd{3.0}{0.1}& - & - & - & - & - & - \\

% {\small \pfMM-\textsc{ELBO}}& \msd{1.0}{0.0} & \bmsd{1.1}{0.0} & \msd{1.6}{0.1} & \msd{1.5}{0.1}& \bmsd{1.1}{0.0} & \bmsd{1.1}{0.1} & \bmsd{1.8}{0.1} & \bmsd{1.7}{0.1} & \bmsd{3.1}{0.1} & \bmsd{2.7}{0.1} \\

% {\small \textsc{Pred-Only}}& \msd{1.0}{0.0} & \bmsd{1.1}{0.0} & \bmsd{1.1}{0.1} & \bmsd{1.0}{0.1}& - & - & - & - & - & - \\
% \bottomrule
% \end{tabular}
% \caption{Mean and (SD) RMSE of the target across 10 boostrap evaluations on the heldout test set. The first level varies the input dimension, the second level varies the number of relevant dimensions and the third level varies the distance between components means of irrelevant dimensions in the data. Each level becomes harder to predict from left to right. Final models are chosen based on target RMSE on a heldout validation set.}
% \label{tab:results}
% \end{table*}



\begin{table*}[t]
\centering
\begin{tabular}{|l | cc | cc || cc | cc | cc | l|}
\hline
\multicolumn{11}{|c|}{Target Mean and (SD) RMSE Across Different Levels of Misspecification} \\ 
\hline
%  & \multicolumn{4}{|c||}{Total Dimensions, $D$ = 10} & \multicolumn{6}{c|}{Total Dimensions, $D$ = 100} \\
%  \cline{2-11}
% & \multicolumn{2}{|c|}{\drel = 5} & \multicolumn{2}{c||}{\drel = 2} & \multicolumn{2}{c|}{\drel = 50} & \multicolumn{2}{c|}{\drel = 10} & \multicolumn{2}{c|}{\drel = 2} \\
%  & \mugap=6 & \mugap=8 & \mugap=6 & \mugap=8 & \mugap=6 & \mugap=8 & \mugap=6 & \mugap=8 & \mugap=6 & \mugap=8 \\
Relevant Dims out of Total: & \multicolumn{2}{c|}{5 out of 10} & \multicolumn{2}{c||}{2 out of 10} & \multicolumn{2}{c|}{50 out of 100} & \multicolumn{2}{c|}{10 out of 100} & \multicolumn{2}{c|}{2 out of 100} \\
 \cline{1-11}
Component Mean Gap, \mugap: & 6 & 8 & 6 & 8 & 6 & 8 & 6 & 8 & 6 & 8 \\
 \hline
{\small \textsc{\twoGMM}}& \bmsd{0.9}{0.0} & \bmsd{1.1}{0.1} & \msd{3.1}{0.1} & \msd{3.0}{0.1}& \bmsd{1.1}{0.0} & \msd{3.1}{0.1} & \msd{3.1}{0.1} & \msd{3.1}{0.1} & \bmsd{3.1}{0.1} & \msd{3.0}{0.1} \\

 
{\small \textsc{GMM}}& \bmsd{0.9}{0.1} & \msd{3.1}{0.1} & \msd{3.1}{0.1} & \msd{3.0}{0.1}& \bmsd{1.1}{0.1} & \msd{3.1}{0.1} & \msd{3.1}{0.1} & \msd{3.2}{0.1} & \bmsd{3.2}{0.1} & \msd{3.0}{0.1} \\

% {\small \pfGMM-\textsc{AltLB}}& \msd{1.0}{0.0} & \bmsd{1.1}{0.1} & \bmsd{1.2}{0.1} & \msd{1.2}{0.0}& - & - & - & - & - & - \\

{\small \pfGMM-\textsc{\loglike}}& \bmsd{0.9}{0.1} & \bmsd{1.1}{0.1} & \bmsd{1.0}{0.1} & \msd{3.0}{0.1}& - & - & - & - & - & - \\

% {\small \pfGMM-\textsc{ELBO}}& \msd{1.0}{0.0} & \bmsd{1.1}{0.0} & \msd{1.6}{0.1} & \msd{1.5}{0.1}& \bmsd{1.1}{0.0} & \bmsd{1.1}{0.1} & \bmsd{1.8}{0.1} & \bmsd{1.7}{0.1} & \bmsd{3.1}{0.1} & \bmsd{2.7}{0.1} \\

{\small \textsc{Pred-Only}}& \msd{1.0}{0.0} & \bmsd{1.1}{0.0} & \bmsd{1.1}{0.1} & \bmsd{1.0}{0.1}& - & - & - & - & - & - \\
\hline
\end{tabular}
\caption{Mean and (SD) RMSE of the target across 10 bootstrap evaluations on the heldout test set. We \textbf{bold} every RMSE value within 1 SD of the smallest 2-SD interval. The first ``level" varies the number of relevant dimensions and the second ``level" varies the distance between components means of irrelevant dimensions in the data. Each level becomes harder to predict from left to right because the misspecification increases.
\pfGMM is more robust in the face of misspecification -- degrading in performance only when the misspecification is severe (i.e. 2 dimensions out of 100 are relevant) -- while continuing to do well when there is no misspecification. 
}
\label{tab:results}
\end{table*}

==> style/tikzlibrary.bayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      % \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      % \draw[->,#1] (\x) -- (\y) ;%
      \draw[-{Latex}] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

